Theoretical Studies on Quantum Walks with a Time-varying Coin

Quantum walks can reconstruct quantum algorithms for quantum computation, where the precise controls of quantum state transfers between arbitrary distant sites are required. Here, we investigate quantum walks using a periodically time-varying coin both numerically and analytically, in order to explore the controllability of quantum walks while preserving its random nature.

==> eptcsdata.tex <==
\providecommand{\firstpage}{74}
\providecommand{\publicationstatus}{G. Di Molfetta, V. Kendon \& Y. Shikano (Eds.): 9th International\\ Conference on Quantum Simulation and Quantum Walks (QSQW 2020)\\
EPTCS 315, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.315.7}{10.4204/EPTCS.315.7}}
\pdfoutput=1

